Parton Propagation and Fragmentation in QCD Matter

We review recent progress in the study of parton propagation, interaction and fragmentation in both cold and hot strongly interacting matter. Experimental highlights on high-energy hadron production in deep inelastic lepton-nucleus scattering, proton-nucleus and heavy-ion collisions, as well as Drell-Yan processes in hadron-nucleus collisions are presented. The existing theoretical frameworks for describing the in-medium interaction of energetic partons and the space-time evolution of their fragmentation into hadrons are discussed and confronted to experimental data. We conclude with a list of theoretical and experimental open issues, and a brief description of future relevant experiments and facilities.

==> discussion.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%               Discussion                                 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Discussion [AA]} 
\label{sec:discussion}

In this Section, we discuss theoretical and experimental topics 
that cross the borders of the artificial division between
Section~\ref{sec:parton} on parton energy loss and
Section~\ref{sec:prehadron} on prehadron absorption, that challenge
the established wisdom, or that did not find space in the main
exposition. 
It is purposely more speculative than the rest of this
review article, and is intended to stimulate new and deeper 
theoretical and experimental studies of parton propagation and
hadronisation. 

\subsection{How to measure the production time, i.e., the quark life
  time [AA]}  \ \\ 
\label{sec:measuretp}

The models presented in Section~\ref{sec:prehadron} and \ref{sec:parton} 
usually quite well reproduce the experimental results on the
multiplicity ratio $R_M^h$.
Therefore, the multiplicity ratio does not allow to 
clearly disentangle the different mechanisms and contributions
of parton energy loss and of pre-hadron interaction.
Most of the difference in the estimates of the
the prehadron production time quoted Section~\ref{sec:formationtimes},
\begin{align}
  t_{preh} \approx f(z) \frac{z\nu}{\kappa} \ ,
\end{align}
lies in the 
different time scale $\kappa$ advocated in each estimate or model
computation. For example, in the simple estimate \eqref{eq:wangest}
the scale $\kappa_h = m_h/R_h \approx 0.2$~GeV/fm leads to the
rather large $\vev{t_h} \approx 50$ fm, used to justify neglect of
prehadronic interaction in cold nuclei, 
instead of $\vev{t_h} \approx 10$ fm  quoted in the Lund
model estimate, where $\kappa_{str} = 1$~GeV/fm. 
In this second case there would be no justification for
neglecting the interactions of the forming hadron field with the
nucleus.
As the choice of the scale $\kappa$ is a debatable and model-dependent
matter~\cite{Kopeliovich:2003py,Wang:2003aw},
it is very important to look for observables which are able to
distinguish energy loss models and absorption models, or to directly
detect in-medium hadronisation effects in order to measure the
prehadron production time $\vev{t_{preh}}$ (in other words, the parton
life time). 

A set of observables have been suggested to be sensitive to the
different mechanisms involved in the hadronisation process and to its
space-time development. These observables and the corresponding
available data are summarised in Table~\ref{table:absvsenloss}, and
discussed below in detail. In Section~\ref{sec:ptbroad}, a rough
estimate of the prehadron production time scale will be provided. 

\begin{table}
  \centering
  \begin{tabular}{lccccc}
    Observable  & Collision & $\vev{t_{preh}}$ & Experiment & Energy& Ref. \\\hline
    $A$-dependence of $R_M^h$ & DIS &  fails 
      &  HERMES &  27~GeV&~\cite{Accardi:2005mm,Accardi:2006ea} \\
    $\tau$-scaling of $R_M^h$ & DIS & $ \sim R_A $ 
      & HERMES & 12, 27~GeV &~\cite{Accardi:2006qs} \\
    Cronin effect vs. $z_h$ and $\nu$& DIS &  $\sim R_A $ 
      & HERMES & 27~GeV 
      &~\cite{Kopeliovich:2003py,Airapetian:2007vu} \\
    $p_{Th}$-broadening & DIS &  $ \gg R_A$
      & CLAS prel.& 4.5~GeV  &~\cite{Kopeliovich:2006xy} \\
                       & DIS &  $\sim R_A$
      & HERMES prel. & 27~GeV  &~\cite{vanHaarlem:2007kj,Accardiprep} \\
    $\pi_0$ vs. $\eta$ suppression & $Au+Au$ & very long 
      & PHENIX & 200~GeV
      &~\cite{Adler:2006bv} \\\hline
  \end{tabular}
  \caption{Information on prehadron production time (parton
    life time) derived form different observables and compared with the nuclear radius $R_A$.
 The energy refers to the lepton beam in the
    target rest frame for DIS, or the nucleon-nucleon centre-of-mass
    frame for $A+A$ collisions. The results have to be read carefully,
    as the typical kinematics varies with the observable and the
    experiment. 
    }
  \label{table:absvsenloss}
\end{table}


\subsubsection{Mass number dependence}-- 
\label{sec:Adep}
The mass number dependence of the nuclear attenuation $1-R^h_M$
 has been suggested to be an observable sensitive to the different 
mechanisms involved in the hadronisation process. 
In first approximation, one expects $1-R^h_M \propto
A^{2/3}$ in energy loss models because the average energy loss
$\Delta E_q \propto \vev{L_q^2} \propto A^{2/3}$, due to the
Landau-Pomeranchuk-Migdal interference in QCD~\cite{Baier:1996sk}.
On the other hand, in absorption models the survival probability is
proportional to the amount of traversed matter, so that $1-R^h_M
\propto \vev{L_A} \propto A^{1/3}$. Therefore a
simple analysis of the $A$-dependence of $R_M^h$ should clearly disentangle
the different contribution.
Recently, it has been shown that 
this argument fails for absorption models
\cite{Accardi:2005jd,Blok:2005vi,Gallmeister:2007an}. If the  
prehadron were produced always at the $\gamma^*$-quark interaction
point (i.e., $t_{preh}=0$) then $R_M = c \,A^{1/3}$ at all
orders in $A^{1/3}$. However, if we allow for a nonzero $\vev{t_{preh}}$, 
its dimension must be neutralised by the nuclear radius $R_A$,
introducing extra powers of $A^{1/3}$. Quite generally, if the
probability distribution for the prehadron production time
 is finite at $t_{preh}=0$, then $R_M^h \propto A^{2/3} +
\mathcal{O}(A)$, the same power found in energy loss models. 

Then, we may study the {\em breaking} of the $A^{2/3}$ law. To this
purpose, it was proposed in~\cite{Accardi:2005jd} to select a set of targets
$\{A_1,A_2,\ldots,A_n\}$, fix the $z$ bin, 
and perform a fit of the form $1-R^h_M(z) =
c(z) A^{\alpha(z)}$ with $c$ and $\alpha$ free
parameters. Results are presented in terms of $2\sigma$
confidence contours in the $(c,\alpha)$ plane.
As shown in Fig.~\ref{fig:RMplus} left, energy loss
\cite{Accardi:2005mm} and absorption models
\cite{Accardi:2005jd,Accardi:2005mm} 
are indistinguishable. The same holds true
for all $z$ bins. Experimental data are described by an $A^\alpha$
power law with $\alpha=0.61 \pm 0.14$, compatible with $\alpha=2/3$
but excluding $\alpha=1/3$.
Increasing the number of targets and the span in
atomic number does not help in separating the 2 models, either, but clearly
shows a non negligible breaking of the $A^{2/3}$ law at $A \gtrsim
80$~\cite{Accardi:2005jd,Accardi:2005mm,Accardi:2006ea}, see
Fig.~\ref{fig:RMplus} right. 

\begin{figure}[tb]
  \vspace*{0cm}
  \centerline{
  \includegraphics[width=6cm]{figure/fig.z065.eps}
  \includegraphics[width=6cm]{figure/fig.z065.HEAVY.eps} 
  }
  \vspace*{0cm}
 \caption[]{
  {\it Left}: results of the $R_M=cA^\alpha$ fit for \{$He$, $N$, $Ne$, $Kr$\} at
  z=0.65 (solid: absorption; dashed: energy loss; dotted: data
 ~\cite{Airapetian:2003mi}). 
  {\it Right}: computations including only heavy nuclei
  \{$Kr$, $Sn$, $Xe$, $W$, $Au$,$Pb$\}. Plots taken from Ref.~\cite{Accardi:2006ea}
 }
 \label{fig:RMplus}
\end{figure}

\subsubsection{Production time scaling in nDIS} --
\label{sec:scaling}
In Ref.~\cite{Accardi:2006qs} it is conjectured that $R_M$ should not
depend on $z_h$ and $\nu$ separately but should
depend on a combination of them:
\begin{align}
  R_M = R_M\big[\tau(z_h,\nu)\big] \ ,
 \label{eq:RMscaling}
\end{align}
where the scaling variable $\tau$ is defined as
\begin{align}
  \tau & = C\, z_h^\lambda (1-z_h) \nu \ .
 \label{eq:scalingvar}
\end{align}
The scaling exponent $\lambda$ is introduced as a way of
approximating and summarising the scaling behaviour of experimental
data and theoretical models. It can be obtained by a best fit
analysis of data or theoretical computations.
The proportionality constant $C$ cannot
be determined by the fit. 
A possible scaling of $R_M$ with $Q^2$ is not considered in this
analysis because of its model dependence, and because of 
the mild dependence of HERMES data on $Q^2$.
As discussed below, the proposed functional
form of $\tau$, Eq.~\eqref{eq:scalingvar}, is flexible enough to
encompass both absorption models 
and energy loss models. The 2 classes of models are distinguished by 
the value of the scaling exponent: a positive $\lambda \gneqq 0$ is
characteristic of absorption models, while a negative $\lambda \lesssim
0$ is characteristic of energy loss models. Thus, the exponent
$\lambda$ extracted from experimental data can identify in the
experimental data the leading mechanism for hadron suppression in
nDIS.

The scaling of $R_M$ is quite natural in the context of hadron
absorption models
\cite{Bialas:1986cf,Accardi:2002tv,Accardi:2005jd,Kopeliovich:2003py,Falter:2004uc,Gallmeister:2005ad} (Sections~\ref{sec:earlystrings} and
\ref{sec:modernstrings}). Indeed, 
prehadron absorption depends on the
in-medium prehadron path length, which depends solely on
the prehadron production time $\vev{t_{preh}}$ as long as $\vev{t_{preh}}
\lesssim R_A$. As argued in 
Section~\ref{sec:formationtimes}, $\vev{t_{preh}} \propto f(z_h) (1-z_h) z_h \nu$
which is well described by the proposed scaling variable $\tau$ with
$\lambda>0$. E.g., in the  Lund model $\lambda \approx 0.7$. 
In energy loss models~\cite{Wang:2002ri,Arleo:2003jz,Accardi:2005mm}
the scaling is 
less obvious, and holds only approximately on a theoretical
ground. When performing the scaling analysis of the full models one
finds in general $\lambda \lesssim 0$~\cite{Accardi:2006qs}. 

\begin{figure}[tb]
  \centering
  \includegraphics[height=6cm,origin=c,clip=true]{figure/fig.lambdafit.eps}
  \includegraphics[height=6cm,origin=t,clip=true]{figure/fig.expdata_27.eps} 
  \caption{{\it Left}: An example of the fit procedure described in
    Section~\ref{sec:scaling}  applied to HERMES data for $\pi^+$
    production on a $Kr$ target~\cite{Airapetian:2003mi}. Upper panel: $\chi^2$ as
    a function of $\lambda$. Lower panel: $R_M(\tau)$ with $\tau$
    computed at $\lambda_{\rm best}=0.34$. {\it Right}: The scaling exponent
    $\lambda_{\rm best}$ extracted from HERMES data on charged and
    identified hadrons at $E_{lab}=27$~GeV
   ~\cite{Airapetian:2000ks,Airapetian:2003mi,Elbakian} 
    (only statistical errors included in
    the fit). Error bars correspond to 1 standard deviation. The bottom
    panel shows the $\chi^2$ per degree of freedom. 
  }
  \label{fig:lambdafit}
\end{figure}

The HERMES experiment measures $R_M$ binned in $z_h$ and integrated
over $\nu$ and $Q^2$ (``$z_h$ distributions'') or binned in $\nu$ and
integrated over $z_h$ and $Q^2$ (``$\nu$ distributions''). 
Eq.~\eqref{eq:RMscaling} is fitted to the combined $z_h$-
and $\nu$-distributions, and the scaling exponent $\lambda$ is
determined by $\chi^2$ minimisation. Note that the scaling variable
is computed using also the measured $\vev{\nu}$ and $\vev{z}$.
An example of this procedure is
illustrated in Fig.~\ref{fig:lambdafit}. Details can be found in
Ref.~\cite{Accardi:2006qs}. 
The scaling exponents $\lambda_{\rm best}$ extracted from HERMES data
at $E_{lab}=27$~GeV~\cite{Airapetian:2000ks,Airapetian:2003mi,Elbakian} 
for different hadron flavours produced on $N$, $Ne$ and $Kr$ targets  
are shown in Fig.~\ref{fig:lambdafit}. In all cases $\chi^2/{\rm
  d.o.f.} \lesssim 1.6$, which proves that $R_M$ scales with $\tau$.
The central result of this analysis is that pion data 
exhibit a clear $\lambda_{\rm best} \approx 0.5 \gneqq 0$. As
discussed, this shows the dominance of the prehadron absorption
mechanism as opposed to the energy loss mechanism, or in other words
is a signal of in-medium prehadron formation, with production times
$\vev{t_{preh}}\lesssim R_A$. 

A similar analysis has been attempted in~\cite{Airapetian:2007vu},
but arbitrarily fixing $\lambda = 0.35$. The resulting $R_M(\tau)$
show a rough scaling, with the 2 lowest-$z_h$ data point in each data
set deviating from the scaling curve and aligning in the vertical
direction. This breaking of the scaling behaviour is more probably 
due to the particular choice of $\lambda$, rather than to rescattering
effects as argued by the authors. 


\subsubsection{$p_T$-broadening and prehadron formation} --
\label{sec:discussion-ptbroad}

The scaling analysis just described 
gives only indirect evidence for a short production time $\vev{t_{preh}}$,
and cannot measure its absolute scale. 
An observable which is more
directly related to the prehadron production time, and allows an
estimate of the coefficient $C$ in Eq.~\eqref{eq:scalingvar}, is the 
hadron's transverse momentum broadening in DIS on a nuclear target
compared to a proton or deuteron target
\cite{Kopeliovich:2003py,Kopeliovich:2006xy},
\begin{align}
  \Delta\vev{p_T^2} = \vev{p_T^2}_A - \vev{p_T^2}_D \ .
\end{align}
When a hadron is observed in the final state, neither the
quark nor the prehadron from which it originates could have had 
inelastic scatterings. Since the prehadron-nucleon elastic 
cross section is very small compared to the quark cross section, 
the hadron's $p_T$-broadening originates dominantly during parton
propagation. As shown in
\cite{Baier:1996sk,Johnson:2000dm}, the quark's momentum
broadening $\Delta p_T^2$ is proportional to the quark path-length
in the nucleus. If the prehadron production time 
has the form \eqref{eq:scalingvar} as argued in the last Section, and
as long as the prehadron is formed inside the nucleus, we obtain 
\begin{align}
  \Delta \vev{p_T^2} \propto \vev{t_{preh}} \propto z^{0.5} (1-z) \nu  \ ,
  \label{eq:ptvsznu}
\end{align}
where the exponent 0.5 is determined by the scaling analysis discussed
in Section \ref{sec:scaling}, and $C$ is to be estimated below.
Then, a decrease of $\Delta p_T^2$ with increasing
$z$ or decreasing $\nu$ would be a clear signal of in-medium prehadron
formation: indeed, if the quark were traveling
through the whole nucleus before prehadron formation, 
$\Delta p_T^2$ would only depend on the nucleus size and not on
$z$ or $\nu$. 
In addition to the dependence of $\Delta\vev{p_T^2}$ on $z$ and
$\nu$, which primarily 
stems from energy conservation and the Lorentz boost of the hadron,
Ref.~\cite{Kopeliovich:2003py} argues that 
\begin{align}
  \Delta \vev{p_T^2} \propto \frac{1}{Q^2} \ .
  \label{eq:ptvsq2}
\end{align}
The physics behind this proposed behaviour is that a quark which is
struck by a photon of large virtuality radiates more intensely than
for a lower virtuality: as a consequence, it will be able to only
travel a shorter way before hadronisation, hence it will experience less
$p_T$-broadening.
A related observable is the Cronin effect, which is likewise expected
to decrease with increasing $z$ 
or decreasing $\nu$, and possibly with increasing $Q^2$
\cite{Kopeliovich:2003py}. 

The HERMES preliminary data on the $p_T$-broadening, see
Figs.~\ref{broad_z_hermes} and \ref{broad_A_hermes},
show a linear increase with $A^{1/3}$, and a clear
decrease of $\Delta\vev{p_T^2}$ at large $z$ consistent with
Eq.~\eqref{eq:ptvsznu} and HERMES data on the Cronin effect
\cite{Airapetian:2007vu}. 
However, HERMES data also show a
clearly increasing $\Delta \vev{p_T^2}$ with $Q^2 = 2-10$~GeV$^2$, which is
at variance with the $Q^2$ dependence of the prehadron production time
\eqref{eq:ptvsq2} obtained in Ref.~\cite{Kopeliovich:2003py}, and an
increase of $\Delta \vev{p_T^2}$ with $x_B$ tending to saturate at
$x_B \gtrsim x_B \gtrsim 0.2$~\cite{Jgoun-prelim}. The flat, or even
slightly decreasing 
dependence of $\Delta\vev{p_T^2}$ on $\nu$ is also, at first sight, 
not easily interpreted in the context of Eq.~\eqref{eq:ptvsznu}
and the simple hadronisation picture used so far. The explanation of
this data set is likely to provide deep theoretical insights on parton
propagation in nuclear matter.

\begin{table}[tb]\centering
\begin{tabular}{|c||c|c|c|c|c|c|}
  \hline
    & $\vev{Q^2}$ [GeV$^2$]
    & $\vev{\nu}$ [GeV]
    & $\vev{z_h}$
    & $\vev{x_B}$
    & $\frac{\vev{Q^2}}{2m_N\vev{\nu}}$
    & $\vev{t_{preh}}$ [fm]\\\hline
  $\vev{\Delta p_{Th}^2}$ vs $A$ & & & & & & \\
  $Ne$ (2.3 fm) & 2.4 & 13.7 & 0.42 & 0.10 & 0.09 & 4.2 \\
  $Kr$ (3.7 fm) & 2.4 & 13.9 & 0.41 & 0.10 & 0.09 & 4.2 \\
  $Xe$ (4.3 fm) & 2.4 & 14.0 & 0.41 & 0.10 & 0.09 & 4.3 \\\hline
  $\vev{\Delta p_{Th}^2}$ vs $z$ 
     & 2.4 & 14.6 & 0.30 & 0.10 & 0.09 &  4.5 \\
     & 2.4 & 13.3 & 0.53 & 0.11 & 0.10 &  3.7 \\
     & 2.3 & 12.6 & 0.74 & 0.11 & 0.10 &  2.3 \\
     & 2.2 & 10.8 & 0.92 & 0.11 & 0.11 &  0.7 \\\hline
  $\vev{\Delta p_{Th}^2}$ vs $\nu$  
     & 2.1 &  8.1 & 0.48 & 0.14 & 0.14 &  2.4 \\ 
     & 2.5 & 12.0 & 0.42 & 0.11 & 0.11 &  3.7 \\
     & 2.6 & 15.0 & 0.40 & 0.10 & 0.09 &  4.6 \\
     & 2.4 & 18.6 & 0.36 & 0.07 & 0.07 &  5.8 \\\hline
  $\vev{\Delta p_{Th}^2}$ vs $Q^2$ 
     & 1.4 & 14.0 & 0.41 & 0.06 & 0.05 &  4.2 \\
     & 2.4 & 14.1 & 0.41 & 0.10 & 0.09 &  4.2 \\
     & 4.5 & 14.5 & 0.39 & 0.18 & 0.16 &  4.3 \\
  \hline
\end{tabular}
\caption{Average HERMES kinematics for the $p_T$-broadening
  results~\cite{vanHaarlem:2007zz,vanHaarlem:2007kj}. 
  In parenthesis, beside the target nucleus symbol is the
  average in-medium path length of the hadronising system 
  $\vev{L_A}\approx (3/4)R_A$, with $R_A=(1.12 \text{\ fm})A^{1/3}$. The
  production time is computed according to Eq.~\eqref{eq:prodtimeest}.
  Note that the average $\vev{x_B}$ is well approximated by
  $\vev{Q^2}/(2m_N\vev{\nu})$. 
  }
\label{tab:HERMESkin}
\end{table}

For a more quantitative interpretation of the data we have first 
to specify the average kinematics in each bin, see
Table~\ref{tab:HERMESkin} and 
Refs~\cite{vanHaarlem:2007zz,vanHaarlem:2007kj}. 
Indeed, different observables and
different experimental bins may be related to different prehadron
production times. In Ref.~\cite{Accardi-prep}, an estimate of the
constant $C$ is obtained from preliminary HERMES based on the
following 2 remarks:
(i) the scaling of $\Delta\vev{p_T^2} \propto
A^{1/3}$ up to the $Xe$ nucleus indicates that the quark path length is
larger than the average in-medium path length $\vev{L_\text{Xe}}$ 
of the hadronising system in the $Xe$ nucleon at $\vev{z} \approx 0.4$,
$\vev{\nu}\approx 14$~GeV, so that the prehadron is always formed on
the surface or outside the nucleus; 
(ii) given the decrease of $\Delta\vev{p_T^2}$ with $z$ as $z\gtrsim
0.5$ the production time at $z\approx 0.4$ fm cannot be much larger
than $\vev{L_\text{Xe}}$. 
Hence, the scale for the production time in
Eq,~\eqref{eq:scalingvar} is
\begin{align}
  C \approx \frac{\vev{L_\text{Xe}}}{\bar z^\lambda (1-\bar z)
    \bar\nu} \approx 0.8 \frac{\text{fm}}{\text{GeV}}
  \label{eq:Cest}
\end{align}
with $\bar z=0.4$ and $\bar\nu=14$~GeV. The average in-medium
path-length of the hadronising system can be approximated as 
$\vev{L_\text{Xe}} \approx (3/4) R_A$ with $R_A = (1.12 
\text{\ fm}) A^{1/3}$, as if nucleons were uniformly
distributed in the nucleus. The resulting production time is
\begin{align}
  \vev{t_{preh}} & \approx  0.8\,  z^{0.5} (1-z) \,\nu \text{\ fm/GeV} \ , 
 \label{eq:prodtimeest}
\end{align}
and it is tabulated in Table~\ref{tab:HERMESkin} for the experimental
bins of interest.
Note that in principle, $C$ should be
allowed to depend on $Q^2$ and $x_B$, but one can neglect it in first
approximation at least for the discussion of the $A$-, $z$-, 
where $\vev{Q^2}$ and $\vev{x_B}$ are rather constant.  

The $\nu$-distribution is also consistent with the estimate
\eqref{eq:prodtimeest}: given the production times in
Table~\ref{tab:HERMESkin},  
it is not surprising that the $\nu$-dependence is basically flat,
because the prehadron is formed outside all the studied nuclei, except
for the first $\nu$-bin. Three effects can contribute to tilt the
curve: 
(i) a possible dependence of the prehadron
cross-section with $\nu$, as it happens for the hadron cross-section;
(ii) medium modifications of the DGLAP parton shower, see
Section~\ref{sec:mDGLAP}, which can modify the linear dependence of
$\Delta\vev{p_T^2}$ on the energy loss $\Delta E$ found in
\cite{Baier:1996sk}, and assumed in Eq.~\eqref{eq:ptvsznu}; 
(iii) the correlation between the $p_T$-broadening and the average
Bjorken variable, $\vev{x_B}$, which will be discussed in detail below. 

We are now in the position to address the intriguing $Q^2$ distribution. 
The linear increase of $\Delta\vev{p_T^2}$ with $Q^2$ is in sharp
contrast with the inverse power dependence from the colour dipole
model. On the other hand also a flat $Q^2$ as would be obtained in most
string-based models, seems at variance with 
these data. However, to our knowledge, no model predicts a substantial
rise of $\vev{t_{preh}}$ with virtuality. How can we explain these data? 
From the production times shown in
Table~\ref{tab:HERMESkin}, we see that the prehadron is always formed
on the surface or outside the nucleus, so that the observed
$Q^2$-dependence must have a partonic origin. It cannot simply come
from multiple parton elastic scatterings, because it would be in first
order proportional to the in-medium parton path-length, which is
basically fixed. Ref.~\cite{Accardi-prep} proposes 3 mechanisms which
can contribute to explain these data:

\begin{enumerate}
\item 
{\it Medium-enhanced DGLAP evolution.}
The scale $Q_0^2$ at which hadronisation
takes place is not expected to strongly depend on the presence of a
medium. Therefore, in the large-$Q^2$ bins, a longer and 
medium-enhanced DGLAP evolution
\cite{Ceccopieri:2007ek,Domdey:2008gp,Borghini:2005em,Armesto:2007dt}
would imply a larger $p_T$-broadening than at low $Q^2$ . 
This mechanism can be investigated with a $\nu > \nu_\text{min}$ cut in
the experimental data: as $\nu_\text{min}$ is increased, 
the DGLAP evolution would increasingly happen outside the nucleus, and
the slope in $Q^2$ should become smaller and smaller. 
\item 
{\it Next-to-leading order processes.}
The basic hard partonic process considered so far is the leading order
(LO) in $\alpha_s$ quark elastic
scattering $\gamma^*+q\ra q$, so that $E_q=\nu$, in the target rest
frame. The next-to-leading order (NLO) gluon fusion process,
$\gamma^*+g \ra q+\bar q$, becomes non-negligible as $x_B$ decreases,
and implies $E_q < \nu$ and a smaller production time.
As can be seen from
Table~\ref{tab:HERMESkin}, the average $\vev{x_B}$ spanned in the
$Q^2$ distribution lies in the transition region between sea partons and
valence quark dominance. Hence, the competition between LO and NLO
process might alter the naive picture of $p_T$-broadening adopted so
far, and lead to its increase with $Q^2$. In this case, the estimate of
$C$ presented in Eq.~\eqref{eq:Cest} would only give a lower limit on the
hadron production time. 
Experimentally, this mechanism can be tested by measuring
$Q^2$-distributions with suitable cuts on $x_B$. 
\item 
{\it Coloured prehadrons with short formation times.}
The prehadron may be produced in a coloured state with a relatively short
production time, but sizeable colour neutralisation time: let's say
\begin{align}
\begin{split}
  \vev{t_{preh}} & \approx 0 \\
  \vev{t_{cn}} & \approx  0.8\,  z^{0.5} (1-z) \,\nu \text{\ fm/GeV} \ .
\end{split}
\end{align}
During the coloured phase, energy loss would lead to
$p_T$-broadening. However, because of colour transparency, the coloured
prehadron may have an inelastic cross section $\sigma_*^\text{inel.}
\propto 1/Q^2$. Hence 
at low $Q^2$ it would be subject to more nuclear absorption than at large
$Q^2$, explaining the linear rise of $\Delta\vev{p_T^2}$ with $Q^2$ 
\footnote{A similar space-time evolution of hadronisation has been
  implemented for leading prehadrons in the GiBUU absorption model of
  Refs.~\cite{Falter:2004uc,Gallmeister:2007an}, which however 
  assumes $t_{preh}=t_{cn}=0$ for leading (but colourless) prehadrons, 
  and does not address radiative energy loss. It
  would be interesting to phenomenologically include both a coloured
  and a colourless prehadron in this model to test the proposed
  scenario.}. 
Note that this scenario does not contradict the dipole model
prediction that $\vev{t_{preh}}\propto 1/Q^2$, but would require the prehadron
to propagate as a coloured state for a time of the order of the nuclear
radius. An experimental investigation of this scenario needs very
large $\nu$, outside the reach of the HERMES experiment but attainable 
at the Electron-Ion Collider (EIC)
\cite{EIChomepage,Deshpande:2005wd}, in order to significantly boost
$\vev{t_{preh}}$ and allow the quark to propagate as a 
free particle inside the nucleus.  
\end{enumerate}
A way studying the physics behind the experimental correlation of
$\Delta\vev{p_T^2}$ with $x_B$ and $Q^2$, is to simultaneously
address $Q^2$-distributions binned in $x_B$ and $x_B$-distributions
binned in $Q^2$, in order to factor out the trivial kinematic
correlation $\nu=Q^2/(2m_Nx_B)$ which affects the production time
\cite{Accardi-prep}.
For example, if $\vev{\tau_p} \propto \nu$, for the LO $\gamma^*+q\ra
q$ scattering we should expect 
\begin{align}
\begin{split}
  Q^{-2}\Delta\vev{p_T^2}_{x_B\text{-bins}} \approx \text{const.} \\
  x_B \Delta\vev{p_T^2}_{Q^2\text{-bins}} \approx \text{const.} 
\end{split}
\end{align}
The deviation from this {\it combined} scaling is going to expose the
underlying dynamics, see Table~\ref{tab:scalingpt2}. 
It is also important to extend as much as possible the range in $x_B$
over which the $p_T$-broadening is measured: at small $x_B\lesssim
0.01$ the NLO photon-gluon fusion is the dominant partonic process,
while at $x_B \gtrsim 0.3-0.4$ the photon dominantly scatter at LO on
valence quarks. Hence, with mechanism number 2, one may expect to
observe a flat $\Delta\vev{p_T^2}$ in these 2 regions. 
Additionally, dihadron correlations and the hadron multiplicity per
event as a function of $x_B$ can more directly reveal the role of NLO
processes, in which 2 partons can be produced at the hard
scattering.

\begin{table}[tb]
\centering
\begin{tabular}{|cc|c|c|}
  \hline
  \multicolumn{2}{|c|}{model} 
    & $Q^{-2}\Delta\vev{p_T^2}_{x_B}$ vs. $Q^2$
    & $x_B \Delta\vev{p_T^2}_{Q^2}$ vs. $x_B$   \\\hline
  $t_{preh}\propto\nu$ 
    & LO                  & $\leftrightarrow$ & $\leftrightarrow$ \\
    & mDGLAP (1)          & $\uparrow$        & $\leftrightarrow$ \\
    & NLO vs. LO (2)      & $\leftrightarrow$ & $\uparrow$        \\
    & coloured $h_c^*$ (3) & $\uparrow$        & $\leftrightarrow$ \\
  $t_{preh}\propto\nu/Q^2$ 
    & colour dipole~\cite{Kopeliovich:2003py} 
                          & $\downarrow$      & $\leftrightarrow$ \\   
  \hline
\end{tabular}
\caption{
  Expected results of the scaling analysis of $p_T$-broadening for
  the models and mechanisms discussed in this paper. The
  numbers in parenthesis refer to the mechanisms listed in
  Section~\ref{sec:Q2xBdist}. The up and down pointing arrows indicate
  increasing or decreasing $p_T$-broadening, the double horizontal
  arrow an approximately constant behaviour.  
  }
\label{tab:scalingpt2}
\end{table}

At CLAS, the kinematics is a bit different due to the lower beam energy,
$E_\text{beam} = 5$~GeV compared to the 27~GeV of HERMES. The main
difference is that $\nu=2-5$~GeV is much smaller than at HERMES,
therefore prehadron production  
should happen on shorter time scales, mainly inside the nucleus according
to the estimate \eqref{eq:ptvsznu}. Note also that $Q^2 = 1-4$, and
that $\vev{x_B}_\text{CLAS} > \vev{x_B}_\text{HERMES}$ at the same
value of the other variables. The preliminary CLAS data
\cite{Hafidi:2006ig,Brooks-Trento,Hicks-Trento} on the $p_T$
broadening and Cronin effect, discussed in Section~\ref{sec:CLASdata},
corroborate the discussed HERMES data
However, the production time we have estimated is about a factor 5
smaller than the production time extracted in
Ref.~\cite{Kopeliovich:2006xy} from preliminary CLAS data on the
$\nu$-dependence of the $p_T$-broadening, see Fig.~\ref{fig:t*fromptbroad}.
The HERMES and CLAS data sets may be qualitatively reconciled if
by taking into account the observed increase of the 
$p_T$-broadening with $x_B$. However, the origin of the discrepancy
between the production times extracted from HERMES and CLAS data on
the $p_T$- broadening remains to be clarified. 
On the theoretical side, the two discussed
methods to determine the production time should be 
applied to both data set, in order to check their
consistency and further explore the issue. On the experimental side,
it is very important to establish and study the correlation of
$\Delta\vev{p_T^2}$ with $x_B$ and $Q^2$, as already emphasised.
 
\begin{figure}[tb]
  \centering
  \includegraphics[width=5cm]{figure/lp.eps}
  \caption{Prehadron production times $\vev{t_{preh}} \equiv l_p$ extracted
    according to Ref.~\cite{Kopeliovich:2006xy} from preliminary CLAS data
   ~\cite{Brooks-JLAB} on $\nu$-distributions of
    $\Delta\vev{p_T}$. Plot taken from Ref.~\cite{Kopeliovich:2006xy}.} 
  \label{fig:t*fromptbroad}
\end{figure}






==> formtimes.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%QCD matter
%%              Formation time estimates                    %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Formation time estimates [AA]}
\label{sec:formationtimes}

As discussed in the introduction, the key quantity we need to
investigate, in order to understand hadron quenching in nuclear
matter, is the quark lifetime, or in other words the hadronisation
time scale. It is the most general information about
the space-time evolution of the hadronisation process which can be
extracted from experimental data. However, hadronisation is a non
perturbative process, and its theoretical understanding is still in
its infancy: one has to resort to phenomenological models to
describe it
\cite{Bialas:1986cf,Accardi:2002tv,Kopeliovich:2003py,Falter:2004uc}.
In this Section, we will discuss the general framework underlying most
models, and some perturbative and non perturbative estimates of
formation times. These ideas will underlie most of the discussion in
Sections \ref{sec:parton} and \ref{sec:prehadron}, where energy loss
and absorption models for parton propagation and hadronisation in
QCD matter will be discussed in detail. 

Even though hadronisation is a non perturbative process, 
a few features can be expected on general grounds.
A parton created in a high-energy collision can travel in the vacuum 
as a free particle only for a limited time because of colour
confinement: it has to dress-up in a colour-field of loosely bound
partons, which eventually will evolve into the observed hadron 
wave function.  
The same dressing process can be expected to happen for partons
traveling in cold QCD matter, which lives in the confining phase
of QCD.  
While the naked, asymptotically free, parton has a negligible inelastic
cross section on the surrounding nucleons, the dressed parton is
likely to develop an inelastic cross section of the order of the
hadronic one. Hence, the dressed parton will be subject to nuclear
absorption in a similar way as a fully formed hadron is. For this
reason, we call it a ``prehadron'', and denote it by $h_*$. 
The prehadron may still be
in a coloured state, since colour neutrality is only requested for the
final state hadron. However, it is likely to neutralise its colour
before hadron formation. We can therefore identify 3 relevant time
scales, see Fig.~\ref{fig:hadrosketch}: 
(1) the ``prehadron production time'' or ``quark lifetime''
$t_{preh}$, at which the dressed quark develops an inelastic cross section,
(2) the ``colour neutralisation time'' $t_{cn}$, at which gluon
brehmsstrahlung stops, and (3) the ``hadron formation time'' $t_h$, at
which the final hadron is formed. 
Note that in a deconfined nuclear medium such as the QGP, the dressing
process may be delayed until the medium cools down and comes closer to
the confinement phase transition. Therefore the struck parton may live
longer in hot QCD matter than in cold QCD matter. 
It is the goal of this review article to
discuss the theoretical and experimental means to determine these
times cales and to understand the underlying physical processes.

For practical applications, hadronisation is generally
pictured as a 2 step process in which the production and colour
neutralisation times are identified, $t_{preh}=t_{cn}$, and sometimes
referred to as the prehadron formation time: the struck quark 
neutralises its colour at once, say by picking up an antiquark from the
vacuum or the surrounding medium and gluon bremsstrahlung stops; the
ensuing colour neutral prehadron quickly develops an inelastic cross
section and at a time $t_h$ its wave function collapses on the wave
function of the observed 
hadron $h$. This is a somewhat crude approximation of the more complex
process sketched above, but is adequate to the present status of the
theoretical and experimental investigation. The possibility that a
prehadron is formed in a state other than a colour singlet will need to
be considered at a more mature stage of the development of theoretical
models. A final caveat is in order: in field theory, it is difficult
to rigorously define the concept of production or formation
time, so that in this review they are used as a phenomenological
working tool.  

\begin{figure}[tb]
  \centering
  \includegraphics[width=10cm]{figure/hadronization.eps}
  \caption{Sketch of the time evolution of the hadronisation process
    with definition of the relevant time scales. A quark $q$ created at
    time 0 in a hard collision turns into a coloured prehadron $h_*^c$,
    which subsequently neutralises its colour, $h_*^0$, and collapses on the
    wave function of the observed hadron $h$.}
  \label{fig:hadrosketch}
\end{figure}

Let us start by estimating the hadron formation time.
A simple estimate can be obtained by defining the average hadron
formation time $\vev{t_h}$ as the time for the 
struck partons to build up its colour field and to develop the
hadronic wave function \cite{Dokshitzer:1991wu}. 
In the hadron rest frame this time is related
to the hadron radius, and in the laboratory frame it is boosted to:
\begin{align} 
  \vev{t_h} \propto R_h \frac{E_h}{m_h} = R_h \frac{z \nu}{m_h}
 \label{eq:wangest}
\end{align}
Note that the scale for hadron formation is set by $\kappa_h = m_h/R_h
\approx 0.2$ GeV/fm.
For a typical 7 GeV pion at HERMES and RHIC, we have $\vev{t_\pi}
\approx 35$ fm $\gg R_A$, which points towards a long quark lifetime
with hadron formation outside the medium. However, for kaons and
protons we obtain much shorter formations times $t_K \approx t_{preh}
\approx 8$ fm, which is comparable to the size of the medium.

\begin{figure}[tb]
  \centering
  \includegraphics[height=3cm]{figure/form-time-pert-1.eps}
  \includegraphics[height=3cm]{figure/form-time-pert-2.eps}
  \caption{Quark hadronisation by emission of 1 parton (left) and
    emission of 1 parton accompanied by many soft gluons (right).}
  \label{fig:pertformtime}
\end{figure}

A more detailed estimate \cite{Vitev05,Adil:2006ra} can be obtained by
looking at hadronisation in light-cone coordinates, where 
for any 4-vector $a^\mu$, we write $a^\mu=(a^+,a^-,\vec a_T)$ with
$a^\pm = (a^0\pm a^3)/\sqrt 2$ and $\vec a_T = (a^1,a^2)$. 
We consider a relativistic on-shell quark of mass $M_q$ and
plus-momentum $p^+$, hadronising into a hadron
of mass $m_h$ and 4 momentum $p_h^+ = z p^+$.
Minimally, hadronisation proceeds by emission of an additional,
typically light, parton to carry away the extra colour, see
Fig.~\ref{fig:pertformtime} left. The process in momentum space is
\begin{align}
  \left[ p^+,\frac{M_q^2}{2p^+},\vec 0_T \right] 
    \lora \left[ z p^+,\frac{m_h^2+\vec k^2}{2 z p^+},\vec k \right] 
    + \left[ (1-z) p^+,\frac{\vec k^2}{2 (1-z) p^+}, - \vec k \right]
 \label{eq:pertproc}
\end{align}
where we imposed 4-momentum conservation. In time-ordered
perturbation theory, the light-cone separation $\Delta y^+$ 
between the initial and final state can be estimated by the 
uncertainty principle: 
\begin{align}
  \Delta y^+ \approx 1/\Delta p^- =  
    \frac{2z(1-z)p^+}{\vec k^2 + (1-z)m_h^2 -z(1-z)M_q^2} \ ,
 \label{eq:pertestimate}
\end{align}
where $\Delta p^- = p^-_{q'} + p^-_h - p^-_q$. The hadron formation
time is then 
\begin{align}
  \vev{t_h} \approx \sqrt{2} \Delta y^+ \ . 
 \label{eq:thpertest}
\end{align}
This estimate should actually be considered an upper limit.
Indeed, hadronisation is a non
perturbative process, hence it will be accompanied by the emission of many
soft gluons, see Fig.~\ref{fig:pertformtime} right. The system of
emitted parton plus soft-gluons has an invariant mass $m_X^2$.  
Taking this into account, we should add an
additional $z m_X^2$ term at the denominator of
Eq.~\eqref{eq:pertproc}, which would reduce the formation time.
In Table~\ref{table:pertformtime} we show the hadron
formation time estimated by Eq.~\eqref{eq:pertestimate} for typical
hadrons at HERMES ($z\approx0.5$, $p^+ \approx \nu \approx 14$ GeV)
and typical mid-rapidity hadrons at RHIC ($z p^+ \approx p_T^h \approx
7$ GeV), where we assumed $\vec k^2 \approx \Lambda_{QCD}^2$. 
As in the previous estimate, pions are formed outside
the medium, kaons and protons have formation times comparable to the
medium size, and heavy flavours are produced pretty quickly inside the
medium.

\begin{table}[tb]
  \centering
  \begin{tabular}{lccccc} 
           & $\pi$ & K        & p    & D      & B      \\\hline
    HERMES & 36 fm & 11 fm    & 3.8 fm   & 1.3 fm & 0.2 fm \\
    RHIC   & 26 fm & 10 fm    & 3.8 fm   & 1.5 fm & 0.2 fm \\\hline
  \end{tabular}
  \caption{Perturbative estimate of hadron formation times $\vev{t_h}$ from
    Eq.~\eqref{eq:pertestimate} for typical hadrons at HERMES
    ($z\approx0.5$, $p^+ \approx \nu \approx 13$ GeV) and at RHIC at
    mid-rapidity ($z p^+ \approx p_T^h \approx 7$ GeV).}
  \label{table:pertformtime}
\end{table}

At least for light quarks, these estimates can be used to justify the
computation of hadron quenching in terms of quark-medium interactions
only, as done in radiative energy loss models
\cite{Wang:2002ri,Arleo:2002kh,Gyulassy:2000er}, see
Section~\ref{sec:parton}. However, even if the hadron is fully formed 
outside the nucleus, the colour field which the quark is building up
might start interacting with the medium much earlier. In other words,
the quark lifetime might actually be smaller than in the above
estimates due to the formation of a prehadron, whose production time
we are going to estimate.

\begin{figure}[tb]
  \centering
  \includegraphics[width=6cm]{figure/Lund-string-breakup.eps}
  \hspace*{.5cm}
  \includegraphics[width=6cm]{figure/Lundtimes.eps}
  \caption{{\it Left:} Hadronisation in the Lund string model in the target
    rest frame. {\it Right:} preahdron production time 
    and hadron formation times for pions
    computed in the Lund string model \cite{Accardi:2005jd}.}
  \label{fig:Lundestimate}
\end{figure}

A successful non perturbative model of hadronisation is the Lund string
model \cite{Andersson:1983ia}, see Fig.~\ref{fig:Lundestimate} left.
The confined colour field stretching from the 
struck quark to the rest of the nucleus is modeled as a
string of tension $\kappa_{str} \approx 1$ GeV/fm, and spans the
lightly shaded area in space-time. The prehadron
formation point is identified with the $q\bar q$ pair production point
$C_i$ which breaks the string in smaller pieces \cite{Bialas:1986cf}.
Hadrons are formed at points $P_i$ when a quark and an antiquark at
the endpoint of a string fragment meet. The subscript $i$ indicates
the so-called rank of the produced (pre)hadron, counted from the right
of the figure. Average prehadron production times can be analytically
computed \cite{Bialas:1986cf,Accardi:2002tv,Accardi:2005jd} and have the
following general structure:
\begin{align}
  \vev{t_{preh}} & = f(z_h) (1-z_h) \frac{z_h \nu}{\kappa_{str}} \\
  \vev{t_h} & = \vev{t_{preh}} + \frac{z_h \nu}{\kappa_{str}} \ ,
 \label{eq:lundest}
\end{align}
where $\nu$ is the struck quark energy.
The factor $z_h \nu$ can be understood as a Lorentz boost factor.
The $(1-z_h)$ factor is due to energy conservation: a high-$z_h$ hadron
carries away an energy $z_h\nu$; the string remainder has a small
energy $\epsilon=(1-z_h)\nu$ and cannot stretch farther than
$L=\epsilon/\kappa_{str}$. Thus the string breaking must occur on a
time scale proportional to $1-z_h$. The function $f(z_h)$ 
is a small deformation of $\vev{t_{preh}}$, which can be computed
analytically in the standard Lund model
\cite{Accardi:2005jd,Bialas:1986cf}. 
The resulting pion formation
time scaled by a factor $\nu/\kappa_{str}$ is plotted in
Fig.~\ref{fig:Lundestimate} left. A typical pion produced at
HERMES has $\vev{t_{preh}} \approx 4$ fm $< R_A$ and 
$\vev{t_h} \approx 6-10$ fm $\gtrsim R_A$, with
similar values at RHIC at mid-rapidity RHIC. 
The final hadron is
typically formed at the periphery or outside the nucleus so that its
interaction with the medium is negligible. 
However, the prehadron is formed well inside and can start interacting
with the nucleus.
A detailed space-time analysis of hadronisation in the {\sc pythia/jetset}
Monte Carlo implementation of the Lund string model has been performed
in \cite{Gallmeister:2005ad}, with similar conclusions regarding the
magnitude of the pion prehadron production time.

\begin{figure}[tb]
  \centering
  \parbox[c]{6.9cm}{\includegraphics[width=7cm]{figure/dipole.berger.eps}} 
  \parbox[c]{0.5cm}{\vskip0.4cm \text{\Large $\approx$}} 
  \parbox[c]{5.2cm}{\includegraphics[width=5.5cm]{figure/dipole.model.eps}}
  \caption{{\it Left:} gauge invariant set
    of diagrams for leading hadron formation in $\ell + A$ collisions
    \cite{Berger:1979xz}. {\it Right:} the dipole model
    approximation.}
  \label{fig:perthadronisation}
  \label{fig:dipmodel} 
\end{figure}

In Ref.~\cite{Berger:1979xz,Berger:1979kz,Kopeliovich:2007yv}
the formation of a leading hadron ($z_h
\gtrsim 0.5$) is described in a pQCD
model, see Fig.~\ref{fig:perthadronisation}.
The struck quark radiates a gluon.  The gluon then splits into a
$q\bar q$ pair, and the $\bar q$ recombines with the struck $q$ to
form the leading prehadron, which later on collapses on the hadron
wave function. The cross section
can be computed from the modulus squared of the sum of the 2 gauge
invariant amplitudes shown in the figure. At $z_h \approx 1$, higher
twist effects spoil this simple mechanism for hadronisation. 
The dipole model of Ref.~\cite{Kopeliovich:2003py} approximates the described 
cross section as a convolution of a Gunion-Bertsch radiation cross
section with the gluon splitting plus quark recombination process, see
Fig.~\ref{fig:dipmodel} right. The prehadron is identified with the 
$q \bar q$ pair which includes the struck quark, 
and its production time is identified with the time at which
the gluon becomes decoherent with the struck quark. (We should note
that, strictly speaking, at the production time the struck
quark-gluon system is in an octet state until gluon splitting
occurs; however, in this model, gluon radiation is neglected during
the octet stage). 
The model can compute the probability distribution in the prehadron
production time, see Fig.~\ref{fig:tpdipolemodel}, and the average
$\vev{t_{preh}}$ is 
\begin{align}
  \vev{t_{preh}} \propto (1-z_h) \frac{z_h \nu}{Q^2} \ .
\end{align}
The interpretation of the $1-z_h$ factor is in terms of energy
conservation: the longer the struck quark propagates, the larger its
energy loss; hence to leave most of its energy to a $z_h \ra 1$
hadron, the quark must be short lived.
The scale is set by $\kappa_{dip} = Q^2$. At HERMES, with $Q^2 \approx
10$ GeV/fm, one obtains for pion production $\vev{t_{preh}} \lesssim 5$ fm
at $z_h>0.5$: pre-pions are formed inside the medium. At
RHIC, where $Q^2 \propto p_T^2$, and $z_h \nu \approx p_T$ for
mid-rapidity hadrons, one obtains the counter-intuitive result that 
$\vev{t_{preh}} \propto 1/p_T$: prehadrons are formed the quicker the higher
their transverse momentum \cite{Kopeliovich:2003py,Kopeliovich:2006xy},
typically inside the medium.

\begin{figure}[tb]
  \vspace*{-.2cm}
  \begin{center}
  \includegraphics[width=6cm,origin=c]{figure/w.eps}
  \end{center}
 \vspace*{-0.3cm}
 \caption[]{
   Probability distribution of the prehadron production time
   $t_{preh}\equiv t$ obtained in the colour dipole model. Plot taken from
   Ref.~\cite{Kopeliovich:2003py}.
 \label{fig:tpdipolemodel}
 }
\end{figure}

In summary, there are considerable uncertainties in the theoretical
estimates of the production times, hence of the length of the partonic
phase of the hadronisation process. It is of foremost importance to
establish the scale of $\vev{t_{preh}}$ and its dependence on the kinematic
variables of the scattering process, through a careful analysis of
experimental data and tests of phenomenological models, see
the discussion in Section~\ref{sec:discussion}. It will be the first step
into a deeper and more detailed understanding of the space-time
evolution of the hadronisation process. 





 

